Doubly Stochastic Models: Learning with Unbiased Label Noises and Inference Stability

Random label noises (or observational noises) widely exist in practical machine learning settings. While previous studies primarily focus on the affects of label noises to the performance of learning, our work intends to investigate the implicit regularization effects of the label noises, under mini-batch sampling settings of stochastic gradient descent (SGD), with assumptions that label noises are unbiased. Specifically, we analyze the learning dynamics of SGD over the quadratic loss with unbiased label noises, where we model the dynamics of SGD as a stochastic differentiable equation (SDE) with two diffusion terms (namely a Doubly Stochastic Model). While the first diffusion term is caused by mini-batch sampling over the (label-noiseless) loss gradients as many other works on SGD, our model investigates the second noise term of SGD dynamics, which is caused by mini-batch sampling over the label noises, as an implicit regularizer. Our theoretical analysis finds such implicit regularizer would favor some convergence points that could stabilize model outputs against perturbation of parameters (namely inference stability). Though similar phenomenon have been investigated, our work doesn't assume SGD as an Ornstein-Uhlenbeck like process and achieve a more generalizable result with convergence of approximation proved. To validate our analysis, we design two sets of empirical studies to analyze the implicit regularizer of SGD with unbiased random label noises for deep neural networks training and linear regression.

==> linear-model.tex <==
\newpage
\section{Learning with Unbiased Label Noises}
In this section, we remodel the problem of deep learning under the Stochastic Gradient Least Square estimator with Unbiased Label Noises (SGD-ULN) settings, where we are specifically interested in the induced bias and the effects of implicit regularization to the generalization performances.

\begin{definition}[Learning with Unbiased Label Noises]
A set of vectors $\mathcal{D}=\{x_1,x_2,x_3,\dots,x_N\}$ drawn from the random variable $\mathcal{X}$ and a $d$-dimensional vector $\theta^*\in \mathbb{R}^d$ are given. The response $y_i$ of the neural network $f^*(x)$ to each sample $x_i\in\mathcal{D}$ is defined as
\begin{equation}
    y_i=y_i^*+\varepsilon_i,\ y_i^*=f^*(x_i),\ \mathrm{ and }\  
    %\varepsilon_i\overset{i.i.d}{\sim}\mathcal{D}. \mathrm{ and }\ 
    \mathbb{E}[\varepsilon_i] =0,\ \mathrm{var}[\varepsilon_i]=\sigma^2_i.
\end{equation}
The problem of learning is to estimate a $d$-dimensional vector $\widehat\theta\in\mathbb{R}^d$, which beats the true neural network $f^*(x)$, using the labeled pairs $\{(x_1,y_1),\dots,(x_N,y_N)\}$.
\end{definition}

\begin{definition}[Learning with ULN via OLS] Given a learning task, the Ordinary Least Square (OLS) estimator under Unbiased Label Noises (ULN) is defined as follow.
\begin{equation}
    \widehat\theta_\mathrm{OLS}\gets\underset{\forall\theta\in\mathbb{R}^d}{\mathrm{arg min}}\ \left\{\Tilde{\mathcal{L}}_N(\theta):=\frac{1}{N}\sum_{i=1}^N\Tilde{L}_i(\theta):=\frac{1}{N}\sum_{i=1}^N\left(f(x_i,\theta)-y_i\right)^2\right\}.\label{eq:dols}
\end{equation}
As the loss function in Eq~\ref{eq:dols} is nonconvex and sometimes non-smooth, we consider the OLS estimator $\widehat\theta$ for learning converges to the point with a small tolerable loss, such that
\begin{equation}
% \widehat\theta_\mathrm{SGLS} \in\left\{\theta:
\Tilde{\mathcal{L}}_N(\widehat\theta)=\frac{1}{N}\sum_{i=1}^N\left(f(x_i,\widehat\theta)-y_i\right)^2\leq \mathrm{tol}% \right\},
\end{equation}
where $\mathrm{tol}$ refers to the convergence criterion on the tolerable training loss.
\end{definition}

\subsection{Generalization Performance of OLS with ULN}
In this section, we discuss the generalization performance of OLS estimator under unbiased label noises.

\begin{definition}[Generalizable Measure of Convergence] We here consider the statistical convergence as how close it could learn a $\theta$ that shares similar behavior of $f^*$. Such that, we define the measure of empirical convergence as
\begin{equation}
   \mathcal{L}_N(\theta) :=\frac{1}{N}\sum_{i=1}^N L_i(\theta):= \frac{1}{N}\sum_{i=1}^N\left(f(x_i,\theta)-f^*(x_i)\right)^2\ ,
\end{equation}
where we characterize the average square error of the model responses on every training sample. We further define a generalizable measure for the convergence as
\begin{equation}
    \mathcal{L}(\theta)=\underset{{x\sim\mathcal{X}}}{\mathbb{E}}\left(f(x,\theta)-f^*(x)\right)^2=\underset{{x_i\sim\mathcal{X}}}{\mathbb{E}}\ \mathcal{L}_N(\theta)\ ,
\end{equation}
which characterizes the expected square error for any $x\sim\mathcal{X}$.
\end{definition}

\begin{assumption}[Bounded Variances] We assume variance of the random noises on each sample is well bounded, such that for all $\varepsilon_i$ and $1\leq i\leq N$ there has $\mathrm{var}[\varepsilon_i]=\sigma_i^2\leq M_1^2$, where $M_1$ is a constant.
\end{assumption}

\begin{assumption}[Bounded Responses] We assume the data samples are all well-normalized and the neural network is with bounded outputs through activation, such that for $\forall\theta\in\mathbb{R}^d$ and $x\sim\mathcal{X}$ there has $|f(x,\theta)|\leq M_2$, where $M_2$ is a constant. We further assume that for some positive real $L$ and every integer $k>1$ there has
\begin{equation}
    \mathbb{E}\ \left|(\varepsilon_i (f(x_i,\theta)-f^*(x_i)))^k\right|\leq\frac{1}{2}\mathbb{E}\ (\varepsilon_i (f(x_i,\theta))-f^*(x_i))^2 {L}^{k-2} k!\ .
\end{equation}
With the above assumption in mind, we can use Bernstein inequalities to bound the effects of noise term.
\end{assumption}


\begin{proposition}[Effects of ULN] In a probability higher than $1-\eta$, for any solution of learning $\widehat\theta$, there has
\begin{equation}
\begin{aligned}
      \mathcal{L}_N(\widehat\theta)&=\Tilde{\mathcal{L}}_N(\widehat\theta)
      +\frac{2}{N}\sum_{i=1}^N\varepsilon_i(f(x_i,\widehat\theta)-f^*(x_i))-\frac{1}{N}\sum_{i=1}^N\varepsilon_i^2\\
      &\leq\mathrm{tol} +\frac{4}{N}\sqrt{\mathrm{log}\frac{1}{\eta}\ \sum_{i=1}^N\sigma_i^2 (f(x_i,\theta)-f^*(x_i))^2}
\end{aligned}
\end{equation}
With the assumptions of bounded variance $\sigma_i^2$ and bounded responses $f(x_i,\theta)$ for $1\leq i\leq N$, we can get $0\leq (f(x,\theta)-f(x,\theta^*))^2\leq 4M_2^2$. we could further conclude that $ \mathcal{L}_N(\widehat\theta)\to \mathrm{tol}$ as $N\to\infty$ and the statistical convergence rate is
\begin{equation}
    \mathcal{L}_N(\widehat\theta)\leq\mathrm{tol}+8M_1M_2\sqrt{ \frac{\mathrm{log}\ 1/\eta}{N}},
\end{equation}
in a probability higher than $1-\eta$.
\end{proposition}

\begin{proposition}[Statistical Convergence under ULN] As $|f(x,\theta)|\leq M_2$ for any $x$ and $\theta$, we can get $0\leq (f(x,\theta)-f(x,\theta^*))^2\leq 4M_2^2$. In this way, we can extend Hoeffiding's inequality to
\begin{equation}
\mathbb{P}\left(\mathcal{L}(\theta)-\mathcal{L}_N(\theta)\geq t\right)\leq\mathrm{exp}\left(-\frac{Nt^2}{8M_2^4}\right)
\end{equation}
%With the assumptions of bounded variance $\sigma_i^2$ and bounded responses $f(x_i,\theta)$ for $1\leq i\leq N$, we could conclude that $\frac{1}{N}\sum_{i=1}^N\left(f(x_i,\theta)-f^*(x_i)\right)^2\to \mathrm{tol}$ as $N\to\infty$ and the statistical convergence rate is
Thus, for any solution of learning $\widehat\theta$, there has
\begin{equation}
    \mathcal{L}(\widehat\theta)\leq\mathrm{tol}+\left(8M_1M_2+2\sqrt{2}M_2^2\right)\sqrt{\frac{\mathrm{log}\ 1/\eta}{N}}\ .
\end{equation}
in a probability higher than $1-2\eta$.
\end{proposition}
\begin{remark} We can conclude that for any $\forall\theta\in\mathbb{R}^d$ there has
$\mathcal{L}_N(\theta)\to\mathcal{L}(\theta),\ \mathrm{ as }\ N\to\infty$.
For the solution of learning $\widehat\theta$ (and $\mathcal{L}_N(\widehat\theta)\leq \mathrm{tol}$), there has
$    \mathcal{L}(\widehat\theta)\leq\mathrm{tol}+\mathcal{O}(\sqrt{1/N})$.
\end{remark}


\section{An Example of Stochastic Gradient based OLS with Unbiased Label Noises}
This section reviews the OLS estimator for linear models with unbiased label noises.
\begin{definition}[Linear Regression with Unbiased Label Noises]
To build a linear model for the regression task, a set of $d$-dimensional vectors $\mathcal{D}=\{x_1,x_2,x_3,\dots,x_N\}$ and a $d$-dimensional vector $\beta^*\in \mathcal{C}$ are given, where $\mathcal{C}$ refers to a set of vectors constraining the structure of the projection. The response $y_i$ of the linear model to each sample $x_i\in\mathcal{D}$ is defined as
\begin{equation}
    y_i=y_i^*+\varepsilon_i,\ y_i^*=x_i^\top\beta^*,\  \mathrm{ and }\  %\varepsilon_i\overset{i.i.d}{\sim}\mathcal{D}
    %\ \mathrm{ and }\ 
    \mathbb{E}[\varepsilon_i] =0,\ \mathrm{var}[\varepsilon_i]=\sigma^2_i,
\end{equation}
where $\varepsilon_i$ refers to a zero-mean random variable with variance $\sigma^2_i$. The problem of linear regression is to estimate a $d$-dimensional vector $\widehat\beta\in\mathcal{C}$, which beats the true parameter $\beta^*$, using the labeled pairs $\{(x_1,y_1),\dots,(x_N,y_N)\}$.
\end{definition}

\begin{definition}[Ordinary Least Square Estimator] Given a linear regression task, the OLS estimator is defined as follow.
\begin{equation}
    \widehat\beta_\mathrm{OLS}\gets\mathrm{arg min}_{\forall\beta\in\mathcal{C}}\ \frac{1}{N}\sum_{i=1}^N\left(x_i^\top\beta-y_i\right)^2.\label{eq:ols}
\end{equation}
Given the matrix $X=[x_1,x_2,\dots,x_N]^\top$ and $Y=[y_1,y_2,\dots,y_N]^\top$, the matrix form of OLS should be as follow.
\begin{equation}
    \widehat\beta_\mathrm{OLS}\gets\mathrm{arg min}_{\forall\beta\in\mathcal{C}}\
    \frac{1}{N}\left\|X\beta - Y\right\|_2^2.\label{eq:mols}
\end{equation}
As the loss function in Eq~\ref{eq:mols} is a strongly smooth and strongly convex, it is not difficult to obtain the solution as the global optimum such that
\begin{equation}
    \nabla\left\|X\beta - Y\right\|_2^2= 0,
\end{equation}
when $\mathcal{C}=\mathbb{R}^d$. In this way, the OLS estimator for linear regression should be
\begin{equation}
    \widehat\beta_\mathrm{OLS} = (X^\top X)^{-1}X^\top Y\ ,
\end{equation}
where $N\gg d$ -- the number of dimensions is much smaller than the number of samples.
\end{definition}

\begin{proposition}[Consistency of OLS-ULN] Suppose the true response $y_i^*$ for the every sample are known. We write the matrix $Y^*=[y_1^*,y_2^*,\dots,y_N^*]^\top$ and the oracle estimate of $\beta^*$ should be as follow,
\begin{equation}
 X\beta^*=Y^*\ \Rightarrow \ \beta^*=(X^\top X)^{-1}X^\top Y^*.
\end{equation}
Let $\epsilon=[\varepsilon_1,\varepsilon_2,\dots,\varepsilon_N]^\top$ and $\mathbb{E} [\epsilon] =[0,\dots,0]^\top=\mathbf{0}_d$, the expected statistical error of $\widehat\beta_\mathrm{OLS}$ to the oracle model should be as follow.
%\begin{equation}
%    \widehat\beta_\mathrm{OLS}-\beta^*=(X^\top X)^{-1}X^\top (Y-Y^*)=(X^\top X)^{-1}X^\top\epsilon.
%\end{equation}
%Thus, the bias of high-dimensional OLS should be
\begin{equation}
    \mathbb{E}\left(\widehat\beta_\mathrm{OLS}-\beta^*\right)=(X^\top X)^{-1}X^\top\mathbb{E}[\epsilon]=\mathbf{0}_d
\end{equation}
OLS thus is a consistent estimator of $\beta^*$. 
\end{proposition}

%\begin{proposition}[Random Matrix and Convergence] We consider $\Sigma_N=\frac{1}{N}X^\top X$ as the covariance matrix of $\{x_1,\dots,x_N\}$. When $N/d\to\infty$, some random matrix theory suggest there exists a constant $K$ that $1/K\leq\lambda_\mathrm{min}(\Sigma_N)\leq \lambda_\mathrm{max}(\Sigma_N) \leq K$. Let $\Theta_N=\Sigma_N^{-1}$. Then $1/K\leq\lambda_\mathrm{min}(\Theta_N)\leq \lambda_\mathrm{max}(\Theta_N) \leq K$. In this way, the statistical convergence rate of $\widehat\beta_\mathrm{OLS}$ to the oracle model should be as follow.
%\begin{equation}
%\begin{aligned}
%    \left\|\widehat\beta_\mathrm{OLS}-\beta^*\right\|_2\leq\frac{1}{N}\left\|(\frac{1}{N}X^\top X)^{-1}\right\|_2\left\|X^\top\epsilon\right\|_2&\leq \frac{K}{N}\left\|X^\top\epsilon\right\|_2
%\end{aligned}
%\end{equation}
%Suppose every sample $x_i$ is well-normalized and consider some matrix concentration inequalities, we could roughly obtain $\|X^\top\epsilon\|\leq\mathcal{O}(\sqrt{dN})$ in high probability. Then, we could obtain the upper bound of convergence as
%\begin{equation}
%    \left\|\widehat\beta_\mathrm{OLS}-\beta^*\right\|_2\leq\mathcal{O}\left(\%sqrt{\frac{d}{N}}\right).
%\end{equation}
%\end{proposition}

%Later we consider the optimization of OLS estimator and its properties.

\subsection{Implicit Regularization of SGD-OLS Estimator with Unbiased Label Noises}
This section presents a simple discussion on the implicit regularization effects of SGD-OLS estimator with unbiased label noises.
\begin{definition}[Stochastic Gradients of OLS-ULN] With mini-batch sampling, SGD algorithm randomly draws a batch of sample $B_t\subseteq\mathcal{X}$ and estimates an stochastic gradient as follow
\begin{equation}
\begin{aligned}
    \Tilde{\mathrm{g}}_t(\beta)
    & = \frac{1}{N}X^\top\left(X\beta-Y^*\right) +\xi_{t}^\mathrm{SGD}(\beta)+\xi_t^\mathrm{ULN}(\beta),
\end{aligned}
\end{equation}
where
\begin{equation}
\begin{aligned}
\xi_\mathrm{t}^\mathrm{SGD}(\beta)&=\left(\frac{1}{|B_t|}\ \sum_{i=1}^{|B_t|} x_i(x_i^\top\beta-y_i^*)-\frac{1}{N}\ \sum_{i=1}^N x_i(x_i^\top\beta-y_i^*) \right),\ \mathrm{and}\\
\xi_\mathrm{t}^\mathrm{ULN}(\beta)&=-\frac{1}{|B_t|}\ \sum_{i=1}^{|B_t|} \varepsilon_ix_i\ .
\end{aligned}
\end{equation}
\end{definition}
\begin{remark}
In this way, we can interpret the stochastic gradient of SGD for OLS estimator with unbiased label noises as three parts as follow,
\begin{itemize}
    \item $\frac{1}{N}X^\top\left(X\beta-Y^*\right)$ - a deterministic gradient term that minimizes the true OLS loss $\frac{1}{N}\|X\beta-Y^*\|_2^2$, 
    \item $\xi_\mathrm{t}^\mathrm{SGD}(\beta)$ - a mini-batch SGD noise term that adapts to $\beta$ and the covariance of gradients of the true loss $\frac{1}{N}\|X\beta-Y^*\|_2^2$, such that
    \begin{equation}
    \begin{aligned}
        \mathbb{E}[\xi_\mathrm{t}^\mathrm{SGD}(\beta)] & = \mathbf{0}_d, \\
        \mathrm{var}[\xi_\mathrm{t}^\mathrm{SGD}(\beta)] & = \mathrm{COV}(\frac{1}{|B_t|}\ \sum_{i=1}^{|B_t|} x_i(x_i^\top\beta-y_i^*)). \label{eq:ols-sgd-noise}
    \end{aligned}
    \end{equation}
    \item $\xi^\mathrm{ULN}_t(\theta)$ - an unbiased gradient noise term caused by label noises $\varepsilon_i$, where to simplify our research we assume $\sigma_1=\sigma_2\dots\sigma_N=\sigma$ then we have
        \begin{equation}
        \begin{aligned}
            {\mathbb{E}}[\xi^\mathrm{ULN}_{t}(\theta)]&=\frac{1}{N}\sum_{i=1}^N\mathbb{E}[\varepsilon_i]\cdot x_i= \mathbf{0}, \\ \mathrm{var}[\xi^\mathrm{ULN}_{t}(\theta)]&=\frac{\sigma^2}{N}\sum_{i=1}^Nx_ix_i^\top\ . %=\sigma^2\nabla\mathcal{L}_N(\theta)\ .
        \end{aligned}
        \label{eq:nlb-noise}
    \end{equation}

    
\end{itemize}
Note that $\mathbb{E}[\Tilde{\mathrm{g}}_t(\beta)]=\mathcal{L}^(\beta)$, the noise would not induce any bias to the gradient estimate of the true loss.
\end{remark}





\begin{remark}
In this way, we can interpret the stochastic gradient of SGD-ULN in three parts as follow
\begin{itemize}
    \item $\nabla\mathcal{L}_N(\theta)$ - a gradient term that minimizes the true square loss $\mathcal{L}(\theta)$, 
    \item $\xi^\mathrm{SGD}_{k}(\theta)$ - a mini-batch SGD noise term that adapts to $\theta$ and the covariance of gradients of the noiseless loss $\mathcal{L}_N(\theta)$, 
    \begin{equation}
    \begin{aligned}
        {\mathbb{E}}[\xi^\mathrm{SGD}_{k}(\theta)] &= \mathbf{0},\\
        \mathrm{var}[\xi^\mathrm{SGD}_{k}(\theta)] &=\Sigma^\mathrm{SGD}(\theta),\  \mathrm{ and}\\  \Sigma^\mathrm{SGD}(\theta) &=\frac{1}{N}\sum_{i=1}^N(\nabla L_i(\theta)-\nabla\mathcal{L}_N(\theta))(\nabla L_i(\theta)-\nabla\mathcal{L}_N(\theta))^\top,
    \end{aligned}
    \label{eq:sgd-noise}
    \end{equation}
    \item $\xi^\mathrm{ULN}_k(\theta)$ - an unbiased gradient noise term caused by label noises $\varepsilon_i$, where to simplify our research we assume $\sigma_1=\sigma_2\dots\sigma_N=\sigma$ then we have
        \begin{equation}
        \begin{aligned}
            {\mathbb{E}}[\xi^\mathrm{ULN}_{k}(\theta)]&=\frac{1}{N}\sum_{i=1}^N\mathbb{E}[\varepsilon_i]\cdot\nabla f(x_i,\theta) = \mathbf{0}, \\ \mathrm{var}[\xi^\mathrm{ULN}_{k}(\theta)]&=\Sigma^\mathrm{ULN}(\theta),\ \mathrm{ and}\\   
            \Sigma^\mathrm{ULN}(\theta)&=\frac{\sigma^2}{N}\sum_{i=1}^N\nabla f(x_i,\theta)\nabla f(x_i,\theta)^\top\ . %=\sigma^2\nabla\mathcal{L}_N(\theta)\ .
        \end{aligned}
        \label{eq:nlb-noise}
    \end{equation}
    
    %, and
    %is independent with $\theta$. Intuitively, the noise term would let the algorithm memorize more about the sample with higher noise.  
\end{itemize}
Note that $\mathbb{E} [\xi_{k}^\mathrm{SGD}(\theta)+\xi_k^\mathrm{ULN}(\theta)] =\mathbf{0}_d$ and $\mathbb{E}[\Tilde{\mathrm{g}}_k(\theta)]=\mathcal{L}_N(\theta)$, the noise would not induce any bias to the gradient estimate of the true square loss.
\end{remark}

\begin{proposition}[Continuous-time dynamics of SGD-ULN] With the step size $\alpha_k=\alpha$ small enough, SGD-ULN estimator would diffuse, in a weak convergence, to its continuous-time limit, such that
\begin{equation}
\begin{aligned}
   \mathbf{d} \theta^\mathrm{ULN}(t) = - \nabla L_N(\theta^\mathrm{ULN}(t))\ \mathbf{d}t &+\sqrt{\frac{\alpha}{B}}\Sigma^\mathrm{SGD}(\theta^\mathrm{ULN}(t)))^{1/2}\ \mathbf{d} W_1(t)\\
   & + \sqrt{\frac{\alpha}{B}}\Sigma^\mathrm{ULN}(\theta^\mathrm{ULN}(t))^{1/2}\ \mathbf{d} W_2(t), \\
   \label{eq:diffuse}
\end{aligned}
\end{equation}
where $t\geq 0$ refers to the time, $W_1(t)$ and $W_2(t)$ refer to standard Brownie motions and $(\cdot)^{1/2}$ as the cholesky decomposition of the matrix. We consider 
$$\sqrt{\frac{\alpha_t}{B}}\Sigma^\mathrm{SGD}(\theta^\mathrm{ULN}(t))^{1/2}\mathbf{d} W_1(t)+\sqrt{\frac{\alpha_t}{B}}\Sigma^\mathrm{ULN}(\theta^\mathrm{ULN}(t))^{1/2}\ \mathbf{d} W_2(t)$$
as an implicit regularization term of the SGD-ULN with unbiased noises.
\end{proposition}

\begin{proposition}[SGD with Noiseless Labels] Let consider an SGD learner over the noiseless loss $\mathcal{L}_N(\theta)$, such that the $k^{th}$ iteration of SGD algorithm picks up a random batch of data $B_t\subseteq\mathcal{D}$ and the algorithm behaves as
\begin{equation}
    \theta_{k+1}\gets\theta_k-\alpha_k\left(\frac{1}{|B_k|}\sum_{i=1}^{|B_t|}(f(x_i,\theta)-f^*(x_i))\cdot\nabla f(x_i,\theta)\right)\ .
\end{equation}
With the step size $\alpha_k$ small enough, such SGD algorithm based on noiseless loss would diffuse, in a weak convergence, to its continuous-time limit, such that
\begin{equation}
\begin{aligned}
   \mathbf{d} \theta^\mathrm{SGD}(t) = & - \nabla \mathcal{L}_N(\theta^\mathrm{SGD}(t))\ \mathbf{d}t%\\ 
   %& 
   +\sqrt{\frac{\alpha}{B}}\Sigma^\mathrm{SGD}(\theta^\mathrm{SGD}(t))^{1/2}\ \mathbf{d} W(t)\ .
   %, \\Q(\theta) & = \left(\+\Sigma^\mathrm{ULN}(\theta)\right)^{1/2}, 
   \label{eq:sgd-noiseless}
\end{aligned}
\end{equation}
We can see an implicit regularization term $\sqrt{\frac{\alpha}{B}}\Sigma^\mathrm{SGD}(\theta^\mathrm{SGD}(t))^{1/2}\ \mathbf{d} W(t)$ contributed by SGD mini-batch sampling in the SDE.
%where $W(t)$ refers to the standard Brownie motion and $(\cdot)^{1/2}$ as the cholesky decomposition of the matrix. %We consider %$$\sqrt{\frac{\alpha_t}{|B_t|}}\left(\Sigma^\mathrm{SGD}(\theta^\mathrm{ULN}(t))+\Sigma^\mathrm{ULN}(\theta^\mathrm{ULN}(t))\right)^{1/2}\ \mathbf{d} W(t)$$ as an implicit regularization term of the SGD-ULN with unbiased noises.
\end{proposition}


\begin{proposition}[Euler Discretization of Two Dynamics] We also consider yet another version of SGD-ULN and SGD algorithms in a format of Euler discretization, such that
\begin{equation}
\begin{aligned}
    \theta_{k+1}^\mathrm{ULN}  = \theta_k^\mathrm{ULN} & - \alpha_k\cdot\nabla L_N(\theta_k^\mathrm{ULN})+\sqrt{\frac{\alpha_k}{|B_k|}}\left(\Sigma^\mathrm{SGD}(\theta_k^\mathrm{ULN})^{1/2} z_k+\Sigma^\mathrm{ULN}(\theta_k^\mathrm{ULN})^{1/2} z'_k\right), \\
    \theta_{k+1}^\mathrm{SGD}  = \theta_k^\mathrm{SGD} & - \alpha_k\cdot\nabla L_N(\theta_k^\mathrm{SGD}) +\sqrt{\frac{\alpha_k}{|B_k|}}\Sigma^\mathrm{SGD}(\theta_k^\mathrm{SGD})^{1/2} z_k, 
    \label{eq:euler-dis}
\end{aligned}
\end{equation}
where $z_k,\ z'_k\sim\mathcal{N}(\mathbf{0}_d,I_d)$ independently. %We consider $$\sqrt{\frac{\alpha_t}{|B_t|}}\left(\Sigma^\mathrm{SGD}(\theta(t))+\Sigma^\mathrm{ULN}(\theta(t))\right)^{1/2}\ \mathbf{d} W(t)$$ as an implicit regularization term of the SGD-ULN with unbiased noises while the regularization effects are controlled by (1) the learning rate $\alpha_t$, the batch size $|B_t|$, (2) the variance of unbiased label noises $\sigma^2$, and (3) the fishier information of neural network function $\frac{1}{N}\sum_{i=1}^N\nabla f(x_i\theta)\nabla f(x_i,\theta)^\top$.
\end{proposition}

\begin{remark}
%As  $\Sigma^\mathrm{SGD}(\theta(t))$ and $\Sigma^\mathrm{ULN}(\theta(t))$ are both symmetric positive (semi)-definite (SPD), there has 
%\begin{equation}
%    \lambda_k(\Sigma^\mathrm{SGD}(\theta(t))+\Sigma^\mathrm{ULN}(\theta(t)))\geq\lambda_k(\Sigma^\mathrm{SGD}(\theta(t)))
%\end{equation}
%for $1\leq k\leq d$ and $\lambda_k(\cdot)$ refers to the $k^{th}$ largest eigenvalue. Furthermore, there has
%\begin{equation}
%    \|\left(\Sigma^\mathrm{SGD}(\theta(t))+\Sigma^\mathrm{ULN}(\theta(t))\right)^{1/2} z
%    \|_2\geq \|\Sigma^\mathrm{SGD}(\theta(t))^{1/2} z\|_2,
%\end{equation}
%for $\forall z\sim\mathcal{N}(\mathbf{0}_d,I_d)$. 
We remark that %the strength of regularization effects of SGD-ULN is stronger than common SGD of least square without any label noises. 
the strength of SGD-ULN implicit regularization is attributed as 
\begin{enumerate}
    \item \emph{SGD} Sampling Noises is controlled by the settings of learning rate $\alpha_t$, the batch size $|B_t|$ as well as the covariance matrix of noiseless loss;
    \item \emph{Variance of Unbiased Label Noises} $\sigma^2$ controls the scale of gradient noises contributed by ULN, such that $\xi^\mathrm{ULN}_k(\theta)\approx\sqrt{\alpha_k/|B_k|}\Sigma^\mathrm{ULN}(\theta)^{1/2}z'_k\propto\sigma$;% for $1\leq k\leq d$; 
    \item  Neural Network Fishier $F^\mathrm{NN}(\theta):=\frac{1}{N}\sum_{i=1}^N\nabla f(x_i\theta)\nabla f(x_i,\theta)^\top$ characterizes the stability of inference results of the neural network $f(x,\theta)$ given the parameter $\theta$ on the training samples $x_1,x_2,\dots,x_N$.
\end{enumerate}
With unbiased label noises at certain scale, we remark that SGD-ULN tends to select an ``stable'' solution $\widehat\theta$ that is with a small $\mathrm{trace}(\nabla f(x_,\widehat\theta)\nabla f(x,\widehat\theta)^\top)$. SGD-ULN would escape from an unstable point faster than common SGD with noiseless settings.
%(1)  (2) and (3) 
\end{remark}


==> removed.tex <==

%\vspace{-3mm}
\section{Implicit Regularization Effects to Linear Regression}%\vspace{-3mm}
%The purpose of this section is to validate \textbf{Propositions 1} and \textbf{2} on the doubly stochastic model and investigate how close it reflects the real-world algorithms of SGD with unbiased label noises. 

Above experiments clearly show the use of unbiased label noises in deep neural networks regression tasks could improve the inference stability and hence boost the performance of models through nois-self distillation. We however hope to see how unbiased label noises would influence the trajectories of SGD iterates. Here, we consider a special example of our study using linear regression, where a simple quadratic loss function is considered for OLS, such that
\begin{equation}
   \widehat\beta_\mathrm{OLS} \gets \underset{\beta\in\mathbb{R}^d}{\mathrm{arg min}}\ \left\{ \frac{1}{N}\sum_{i=1}^N\tilde{L}_i(\beta):=\frac{1}{2N}\sum_{i=1}^N\left(x_i^\top\beta-\tilde{y}_i\right)^2\right\}\ ,\label{eq:linear-net}
\end{equation}
where samples are generated through $\tilde{y}_i=x_i^\top\beta^*+\varepsilon_i$, $\mathbb{E}[\varepsilon_i]=0$ and $\mathrm{var}[\varepsilon_i]=\sigma^2$. Note that in this section, we replace the notation of $\theta$ with $\beta$ to present the parameters of linear regression models.


\subsection{Learning Dynamics SGD with Unbiased Label Noises for Ordinary Least Squares}
Let \lxh{}{us} combine Eq.~\eqref{eq:linear-net} and Eq.~\eqref{eq:sgduln}. We write the SGD for Ordinary Least Squares with Unbiased Label Noises as the iterations $\beta_k^\mathrm{ULN}$ for $k=1,2,3\dots$ as follow
    \begin{equation}
    \beta^\mathrm{ULN}_{k+1}\gets\beta^\mathrm{ULN}_k-\frac{\eta}{N}\sum_{i=1}^N\nabla L_i^*(\beta^\mathrm{ULN}_k)+\sqrt{\eta}\xi_k^*(\beta^\mathrm{ULN}_k)+\sqrt{\eta}\xi_k^\mathrm{ULN}(\beta^\mathrm{ULN}_k),
\end{equation}
where $\nabla {L}^*_i(\beta)$ for $\forall\theta\in\mathbb{R}^d$ refers to the loss gradient based on the label-noiseless sample $(x_i,y_i)$ and $y_i=x_i^\top\beta^*$, ~$\xi^*_{k}(\beta)$ refers to stochastic gradient noises caused by mini-batch sampling over the gradients of label-noiseless samples, and $\xi_{k}^\mathrm{ULN}(\beta)$ is an additional noise term caused by the mini-batch sampling and the unbiased label noises, such that
\begin{equation}\label{eq:key-terms}
\begin{aligned}
%\mathcal{L}_N(\theta)&=\frac{1}{N}\sum_{i=1}^N\left(f(x_i,\theta)-f^*(x_i)\right)^2:=\frac{1}{N}\sum_{i=1}^N L_i(\theta)\\
\nabla {L}^*_i(\beta)&=\frac{\partial}{\partial\beta}\frac{(x_i^\top\beta-x_i^\top\beta^*)^2}{2}=x_ix_i^\top(\beta-\beta^*) ,\\
\xi^*_{k}(\beta)&=\frac{\sqrt{\eta}}{|B_k|}\sum_{x_j\in B_k}\left(\nabla L^*_j(\beta) -\frac{1}{N}\sum_{i=1}^NL^*_i(\beta)\right),\\% \text{and }\  \mathbb{E}_{B_k}[\xi^*_{k}(\theta)] = \mathbf{0}_d ,\\
\xi_{k}^\mathrm{ULN}(\beta)&= - \frac{\sqrt{\eta}}{|B_k|}\ \sum_{x_j\in B_k} \varepsilon_j\cdot x_j\ .%,\ \\ %,\ \text{and }\  {\mathbb{E}}_{B_k,\varepsilon_i}[\xi_{k}^\mathrm{ULN}(\theta)]= \mathbf{0}_d  .
\end{aligned}
\end{equation}
%
We denote the \emph{sample covariance matrix} of $N$ samples as 
\begin{equation}
    \bar\Sigma_N=\frac{1}{N}\sum_{i=1}^{N}x_ix_i^\top\ ,
\end{equation}
and then can use the general forms in Eq.~\ref{eq:covariance} to obtain $\Sigma^\mathrm{SGD}(\beta(t))$ and $\Sigma^\mathrm{ULN}(\beta(t))$ as follows,
\lxh{}{
\begin{equation}\label{eq:cov-ols}
%\footnotesize
    \begin{aligned}
        \Sigma_N^\mathrm{SGD}(\beta)&
        =\frac{1}{N}\sum_{i=1}^{N}\left(x_ix_i^\top-
        \bar\Sigma_N\right)(\beta-\beta^*)(\beta-\beta^*)^\top\left(x_ix_i^\top-
        \bar\Sigma_N\right)^\top\\
        &=\mathrm{Var}_i\left[(x_ix_i^\top-\bar\Sigma_N)(\beta-\beta^*)\right],\ \text{and }\ 
        \\
        \Sigma_N^\mathrm{ULN}(\beta)&
        =\mathbb{E}_k\left[\xi_{k}^\mathrm{ULN}(\beta)\xi_{k}^\mathrm{ULN}(\beta)^\top\right]=\frac{\sigma^2}{N}\sum_{i=1}^{N}x_ix_i^\top
        =\sigma^2\bar\Sigma_N\ ,
    \end{aligned}
\end{equation}
where $\mathrm{Var}_i\left[(x_ix_i^\top-\bar\Sigma_N)(\beta-\beta^*)\right]$ refers to the (co-)variance matrix of vectors $(x_ix_i^\top-\bar\Sigma_N)(\beta-\beta^*)$ with varying $x_i$. Apparently the noise term $\xi_{k}^\mathrm{ULN}(\beta(t))$ is independent with the time-varying location of $\beta(t)$ and $\Sigma^\mathrm{SGD}(\beta(t))$ depends on the location of $\beta(t)$. }

We combine \textbf{Proposition 2} and above Equations to obtain the mean and variance of noise vectors as follow
\begin{equation}\label{eq:cov-ols}
    \begin{aligned}
    &\mathbb{E}_{B_k}\ \xi^*_{k}(\beta)  =\mathbf{0_d},\ & \text{and}\ & \mathbb{E}_{B_k}\ \xi^\mathrm{ULN}_{k}(\beta)=\mathbf{0_d}\\
    &\mathrm{Var}_{B_k}\ [\xi^*_{k}(\beta)]=\frac{\eta}{|B_k|}\Sigma_n^\mathrm{SGD}(\beta),\ & \text{and}\ & \mathrm{Var}_{B_k}\ [\xi^\mathrm{ULN}_{k}(\beta)]=\frac{\eta}{|B_k|}\Sigma_n^\mathrm{ULN}(\beta)\ .
    \end{aligned}
\end{equation}


With respect to the general form of continuous-time doubly stochastic model for SGD with unbiased label noises (\textbf{Definition 1}), the continuous-time diffusion processes of SGD algorithms for Ordinary Least-Square (OLS) with and without unbiased label noises could be modeled as follow.
\begin{equation}\label{eq:doublystoch-ols}
%\footnotesize
\begin{aligned}
        \mathbf{d} \beta^\mathrm{ULN}(t)=& -\bar\Sigma_N\left(\beta^\mathrm{ULN}(t)-\beta^*\right) \mathbf{d}t+\sqrt{\frac{\eta}{B}}\Sigma_N^\mathrm{SGD}(\beta^\mathrm{ULN}(t))^{1/2}\mathbf{d} W_1(t) &\\
        &+\sqrt{\frac{\eta\sigma^2}{B}}\bar\Sigma_N^{1/2}\mathbf{d} W_2(t)\\
        \mathbf{d} \beta^\mathrm{LNL}(t)=& -\bar\Sigma_N\left(\beta^\mathrm{LNL}(t)-\beta^*\right) \mathbf{d}t+\sqrt{\frac{\eta}{B}}\Sigma_N^\mathrm{SGD}(\beta^\mathrm{LNL}(t))^{1/2}\mathbf{d} W(t)
    \end{aligned}
\end{equation}
where $\beta^\mathrm{ULN}(t)$ and $\beta^\mathrm{LNL}(t)$ refer to the SGD dynamics for OLS under \underline{U}nbiased \underline{L}abel \underline{N}oises and \underline{L}abel \underline{N}oise\underline{L}ess settings. 
%

In this way, we combine Eqs.~\eqref{eq:doublystoch-ols} and \textbf{Proposition 2}. Correspondingly, when $\mathbf{dt}=\eta$ the discrete-time approximation of above two SDEs should be iterations for $k=1,2,3\dots$ as follows.
\begin{equation}\label{eq:doublystoch-disols}
\begin{aligned}
        \bar\beta^\mathrm{ULN}_{k+1}= \bar\beta^\mathrm{ULN}_{k} -\eta\bar\Sigma_N\left(\bar\beta^\mathrm{ULN}_k-\beta^*\right) &+\frac{\eta}{\sqrt{B}}\Sigma_N^\mathrm{SGD}(\bar\beta^\mathrm{ULN}_k)^{1/2}z_k+\frac{\eta\sigma^2}{\sqrt{B}}\bar\Sigma_N^{1/2} z'_k\\
        \bar\beta^\mathrm{LNL}_{k+1}= \bar\beta^\mathrm{LNL}_{k} -\eta\bar\Sigma_N\left(\bar\beta^\mathrm{LNL}_k-\beta^*\right) &+\frac{\eta}{\sqrt{B}}\Sigma_N^\mathrm{SGD}(\bar\beta^\mathrm{LNL}_k)^{1/2} z_k\ ,
    \end{aligned}
\end{equation}
where $z_k$ and $z'_k\sim\mathcal{N}(\mathbf{0_d},\mathbf{I_d})$ referring to the standard white noises drawn per iteration. Compared to $\beta^\mathrm{LNL}(t)$ and $\bar\beta^\mathrm{LNL}_k$, the dynamics $\beta^\mathrm{ULN}(t)$ and iterations $\bar\beta^\mathrm{ULN}_k$ incorporate additional noise terms $\sqrt{\frac{\eta}{B}}\Sigma_N^\mathrm{ULN}(\beta^\mathrm{ULN}(t))^{1/2}\mathbf{d} W_2(t)$ and $\sqrt{\frac{\eta}{B}}\Sigma_N^\mathrm{ULN}(\bar\beta^\mathrm{ULN}_k)^{1/2}z'_k$ which affect the dynamics and iterations.

\subsection{Implicit Regularization Effects of SGD with Unbiased Label Noises for Ordinary Least Squares}


%\begin{remark}[Implicit Regularization on OLS is Data-Dependent]
We combine \emph{Remark 1} and Eq~\eqref{eq:doublystoch-disols}, and could approximate the implicit regularizer of SGD with the random label noises for OLS through discretization such as,
\begin{equation}
\begin{aligned}
%&\sqrt{\frac{\eta}{B}}\Sigma_N^\mathrm{ULN}(\beta^\mathrm{ULN}(t))^{1/2}\mathbf{d} W_2(t) \\
%& \Rightarrow\    
\xi_k^\mathrm{ULN}(\beta)\approx\left(\frac{\eta\sigma^2}{B}\bar\Sigma_N\right)^\frac{1}{2}z'_k=\left({\frac{\eta\sigma^2}{NB}\sum_{i=1}^Nx_ix_i^\top}\right)^\frac{1}{2}%\left(\bar\Sigma_N\right)^{1/2} 
z'_k,\ \text{and}\ z'_k\sim\mathcal{N}(\mathbf{0}_d,\mathbf{I}_d),\ 
\end{aligned}\label{eq:oup}
\end{equation}
which is unbiased $\mathbb{E}[\xi_k^\mathrm{ULN}(\beta)]=\mathbf{0_d}$ with invariant covariance structure, and is independent with $\beta$ (the location) and $k$ (the time).
%, but is data-dependent (i.e., with $\bar\Sigma_N$).


\lxh{}{To analyze the asymptotic behaviors of SGD with unbiased label noises, we can obtain the solutions of SDE~\eqref{eq:doublystoch-ols} as follow.
\begin{equation}\label{eq:doublystoch-ols-solutions}
\begin{aligned}
\beta^\mathrm{ULN}(t)-\beta^\mathrm{ULN}(0)  =  &  -\int_0^t\bar\Sigma_N\left(\beta^\mathrm{ULN}(s)-\beta^*\right) \mathbf{d} s\\
&+ \sqrt{\frac{\eta}{B}}\int_0^t\Sigma_N^\mathrm{SGD}(\beta^\mathrm{ULN}(s))^{1/2}\mathbf{d} W_1(s)\\
&+ \sqrt{\frac{\eta\sigma^2}{B}}\int_0^t\bar\Sigma_N^{1/2}\mathbf{d} W_2(s)\\ %\ , \ \widehat{\Theta}(0)=\theta_0 \ .
\beta^\mathrm{LNL}(t)- \beta^\mathrm{LNL}(0)  = &  -\int_0^t\bar\Sigma_N\left(\beta^\mathrm{LNL}(s)-\beta^*\right) \mathbf{d} s\\
&+ \sqrt{\frac{\eta}{B}}\int_0^t\Sigma_N^\mathrm{SGD}(\beta^\mathrm{LNL}(s))^{1/2}\mathbf{d} W(s) .
\end{aligned}
\end{equation}}


%Thus, we could obtain the gap between two processes as
%\begin{equation}
%\begin{aligned}
%        \mathbf{d}\left(\beta^\mathrm{ULN}(t)-\beta^\mathrm{LNL}(t)\right)=&-\bar\Sigma_N\left(\beta^\mathrm{ULN}(t)-\beta^\mathrm{LNL}(t)\right)\mathbf{d}t+\sqrt{\frac{\eta}{B}}\left(\sigma^2\bar\Sigma_N\right)^{1/2}\mathbf{d} W(t)\ . 
%\end{aligned}\label{eq:oup}
%\end{equation}
%The solution of SDE in Eq.~\eqref{eq:oup} is identified as an multidimensional \emph{Ornstein-Uhlenbeck} process~\cite{bhattacharya2009stochastic}, which has explicit form as follow
%\begin{equation}
%\begin{aligned}
%    &\left(\beta^\mathrm{ULN}(t)-\beta^\mathrm{LNL}(t)\right)
%    =\sqrt{\frac{\eta\sigma^2}{B}}\int_{0}^t\mathrm{exp}\left(-(t-\tau)\bar\Sigma_N\right)\left(\bar\Sigma_N\right)^{1/2}\mathbf{d} W(\tau)\ ,
%\end{aligned}
%\end{equation}
%when the two dynamics start from the same point $\beta^\mathrm{ULN}(0)=\beta^\mathrm{LNL}(0)$.
%\end{remark}


\lxh{According to~\cite{berthier2020tight}, SGD for noiseless linear regression would asymptotically converge to the optimal solution $\beta^*$. As the additional noise term $\xi^\mathrm{ULN}$ is unbiased with an invariant covariance structure, when $t\to\infty$ the solution of SDE~\eqref{eq:doublystoch-ols} would be $\underset{t\to\infty}{\lim}\mathbb{E}\ \beta^\mathrm{LNL}(t)=\underset{t\to\infty}{\lim}\mathbb{E}\ \beta^\mathrm{ULN}(t)=\beta^*$, $\underset{t\to\infty}{\lim}\mathbf{d}\beta^\mathrm{ULN}(t)=(\frac{\eta\sigma^2}{B}\bar\Sigma_N)^{1/2}\mathbf{d}W_2(t)$. By definition of a distribution from a stochastic process, we could have $\underset{t\to\infty}{\lim}\mathbf{d}\beta^\mathrm{ULN}(t)\to\mathcal{N}(\beta^*,(\frac{\eta\sigma^2}{B}\bar\Sigma_N)^{1/2})$--a stationary distribution.}{}

\begin{remark}  Thus, with $k\to\infty$, the SGD algorithm for OLS with unbiased label noises would converge to a distribution of Gaussian-alike as follow
\begin{equation}
  \lim_{k\to\infty}\mathbb{E}\ [\beta_k^\mathrm{ULN}]=\beta^*, \text{and}\ \lim_{k\to\infty}\mathrm{Var}\ [\beta_k^\mathrm{ULN}] = \frac{\eta\sigma^2}{B}\bar\Sigma_N,
\end{equation}
The span and shape of the distribution are controlled by $\sigma^2$ and $\bar\Sigma_N$ when $\eta$ and $B$ are constant. %Please refer to Appendix A.3 for the proofs.
\end{remark}

%we could conclude that when $k\to\infty$, SGD with unbiased random label noises would converge to a distribution centered at $\beta^*$. The distribution would tend to be a Gaussian distribution when $\sigma^2$ is significant (we could not ignore the effects of stochastic gradient noise terms of noiseless loss to the overall distribution), as the term $\sqrt{\sigma^2\eta/B}\bar\Sigma_N^{1/2}\mathbf{d} W(t)$ corresponds to a Gaussian distribution. 

%the gap between two dynamics $\beta^\mathrm{ULN}(t)-\beta^\mathrm{LNL}(t)$ would not converge to $0$ due to the path integral, while the size of the gap is controlled by $\sigma^2$ and shape (distribution) of the gap would be controlled by $\Sigma_N$, when the learning rate and batch size are fixed.



\begin{figure}
    \subfloat[${\sigma}^2=0.25$]{\includegraphics[width=0.45\textwidth]{SGD-20-0-0-20-0.25.png}}\hfill
    \subfloat[${\sigma}^2=0.5$]{\includegraphics[width=0.45\textwidth]{SGD-20-0-0-20-0.5.png}}\hfill
    \subfloat[${\sigma}^2=1.0$]{\includegraphics[width=0.45\textwidth]{SGD-20-0-0-20-1.png}}\hfill
    \subfloat[${\sigma}^2=2.0$]{\includegraphics[width=0.45\textwidth]{SGD-20-0-0-20-2.png}}\hfill%\vspace{-3mm}
%\end{figure}
%%\vspace{-3mm}
%\begin{figure}
%    \subfloat[$\tilde{\sigma}=1.0$]{\includegraphics[width=0.25\textwidth]{SGD-20-10-10-20-2.png}}\hfill
    \subfloat[$\Sigma_{1,2}=10\cdot\mathbf{I}_d$]{\includegraphics[width=0.45\textwidth]{SGD-10-0-0-10-0.5.png}}\hfill
    \subfloat[$\Sigma_{1,2}=100\cdot\mathbf{I}_d$]{\includegraphics[width=0.45\textwidth]{SGD-100-0-0-100-0.5.png}}\hfill
    \subfloat[$\Sigma_{1,2}=\Sigma^\mathrm{Ver}$]{\includegraphics[width=0.45\textwidth]{SGD-10-0-0-100-0.5.png}}\hfill
    \subfloat[$\Sigma_{1,2}=\Sigma^\mathrm{Hor}$]{\includegraphics[width=0.45\textwidth]{SGD-100-0-0-10-0.5.png}}\hfill
    %\vspace{-3mm}
    \caption{Trajectories of SGD over OLS with and without Unbiased Random Label Noises using various $\tilde{\sigma}^2$ and $\Sigma_{1,2}$ settings for (noisy) random data generation. For Figures~(a)--(d), the experiments are setup with a fixed $\Sigma_{1,2}=[[20,0]^\top,[0,20]^\top]$ and varying $\tilde{\sigma}^2$. For Figures~(e)--(h), the experiments are setup with a fixed $\tilde{\sigma}^2=0.5$ and varying $\Sigma_{1,2}$, where we set $\Sigma^\mathrm{Ver}=[[10,0]^\top,[0,100]^\top]$ and $\Sigma^\mathrm{Hor}=[[100,0]^\top,[0,10]^\top]$ to shape the converging distributions.}
    \label{fig:SGD-OLS}
%\vspace{-5mm}
\end{figure}



\subsection{Numerical Validation with Synthesized Data} To validate above findings in linear regression settings, we carry out numerical evaluation using synthesize data to simply visualize the dynamics over iteration of SGD algorithms with label-noisy OLS and label-noiseless OLS. In our experiments, we use 100 random samples realized from a 2-dimension Gaussian distribution $X_i\sim\mathcal{N}(\mathbf{0},\Sigma_{1,2})$ for $1\leq i\leq 100$, where $\Sigma_{1,2}$ is an symmetric covariance matrix controlling the random sample generation. To add the noises to the labels, we first \lxh{drawn}{draw} 100 copies of random noises from the normal distribution with the given variance $\varepsilon_i\sim\mathcal{N}(0,{\sigma}^2)$, then we setup the OLS problem with $(X_i,\tilde{y}_i)$ pairs using $\tilde{y}_i={X}_i^\top\beta^*+\varepsilon_i$ and $\beta^*=[1,1]^\top$ and various settings of ${\sigma}^2$ and $\Sigma_{1,2}$. We setup the SGD algorithms with the fixed learning rate $\eta=0.01$, and \lxh{bath}{batch} size $B=5$, with the total number of iterations $K=1,000,000$ to visualize the complete paths. %and $\sigma=1$ $\Sigma_{1,2}=[[20,0]^\top,[0,20]^\top]$ and $\sigma=2$



Figure~\ref{fig:SGD-OLS} presents the results of numerical validations. In Figure~\ref{fig:SGD-OLS}(a)--(d), we gradually \lxh{increases}{increase} the variances of label noises $\sigma^2$ from $0.25$ to $2.0$, where we can observe (1) SGD over label-noiseless OLS converges to the optimal solution $\beta^*=[1.0,1.0]^\top$ in a fast manner, (2) SGD over OLS with unbiased random label noises would asymptotically converge to a distribution centered at the optimal point, and (3) when $\sigma^2$ increases, the span of the converging distribution becomes larger. In Figure~\ref{fig:SGD-OLS}(e)--(h), we use four settings of $\Sigma_{1,2}$, where we can see (4) no matter how $\Sigma_{1,2}$ is set for OLS problems, the SGD with unbiased random label noises would asymptotically converge to a distribution centered at the optimal point. 


Compared the results in~(e) with(f), we can find that, when the trace of $\Sigma_{1,2}$ increases, the span of converging distributions would \lxh{increases}{increase}. Furthermore, (5) the shapes of converging distributions depend on $\Sigma_{1,2}$. In Figure~\ref{fig:SGD-OLS}(g), when we place the principal component of $\Sigma_{1,2}$ onto the vertical axis (i.e., $\Sigma^\mathrm{Ver}=[[10,0]^\top,[0,100]^\top]$), the distribution lays on the vertical axis principally. Figure~\ref{fig:SGD-OLS}(h) demonstrates the opposite layout of the distribution, when we set $\Sigma^\mathrm{Hor}=[[100,0]^\top,[0,10]^\top]$ as $\Sigma_{1,2}$. The scale and shape of the converging distribution backups our theoretical investigation in Eq~\eqref{eq:oup}.
%

Note that the unbiased random label noises are added to the labels prior to the learning procedure. In this setting, it is the mini-batch sampler of SGD that re-samples the noises and influences the dynamics of SGD through forming the implicit regularizer.

%independent with $t$ and $\beta$. 


%We then define the data Fisher matrix as 
%\begin{equation}
% F^\mathrm{D}=\frac{1}{N}\sum_{i=1}^Nx_ix_i^\top.   
%\end{equation}
%Then we have $\Sigma^\mathrm{ULN}(\beta)=\sigma^2F^\mathrm{D}$.
%three parts as follow,
%\begin{itemize}
%    \item $\frac{1}{N}X^\top\left(X\beta-Y^*\right)$ - a deterministic gradient term that minimizes the true OLS loss $\frac{1}{N}\|X\beta-Y^*\|_2^2$, 
%    \item $\xi_\mathrm{t}^\mathrm{SGD}(\beta)$ - a mini-batch SGD noise term that adapts to $\beta$ and the covariance of gradients of the noiseless loss $\frac{1}{N}\|X\beta-Y^*\|_2^2$, such that
%    \begin{equation}
 %   \begin{aligned}
 %       \mathbb{E}[\xi_\mathrm{t}^\mathrm{SGD}(\beta)] & = \mathbf{0}_d, \\
 %       \mathrm{var}[\xi_\mathrm{t}^\mathrm{SGD}(\beta)] & = \mathrm{COV}(\frac{1}{|B_t|}\ \sum_{i=1}^{|B_t|} x_i(x_i^\top\beta-y_i^*)). \label{eq:ols-sgd-noise}
 %   \end{aligned}
 %   \end{equation}
 %   \item $\xi^\mathrm{ULN}_t(\theta)$ - an unbiased gradient noise term caused by label noises $\varepsilon_i$, where to simplify our research we assume $\sigma_1=\sigma_2\dots\sigma_N=\sigma$ then we have
 %       \begin{equation}
 %       \begin{aligned}
  %          {\mathbb{E}}[\xi^\mathrm{ULN}_{t}(\theta)]&=\frac{1}{N}\sum_{i=1}^N\mathbb{E}[\vareps%ilon_i]\cdot x_i= \mathbf{0}, \\ \mathrm{var}[\xi^\mathrm{ULN}_{t}(\theta)]&=\frac{\sigma^2}{N}\sum_{i=1}^Nx_ix_i^\top\ . %=\sigma^2\nabla\mathcal{L}_N(\theta)\ .
  %      \end{aligned}
  %      \label{eq:nlb-noise}
  %  \end{equation}

    
%\end{itemize}
%Note that $\mathbb{E}[\Tilde{\mathrm{g}}_t(\beta)]=\mathcal{L}^(\beta)$, the noise would not induce any bias to the gradient estimate of the noiseless loss.
%\end{remark}
%\input{linear-model}


% deep models




% Note that for the symmetric noise and the Gaussian one, the curve is with the best scale of label noises on the validation set.



==> stat-GLM.tex <==

\begin{proposition}[SGD-OLS Estimator]
We consider the term ${R}_N(\beta)$ as an implicit regularizer and rewrite the OLS estimator in \textbf{Definition 2} as follow,
\begin{equation}
    \widehat\beta_\mathrm{OLS}^\mathrm{SGD}\gets\underset{\beta\in\mathbb{R}^d}{\mathrm{arg min}}\ \left\{\frac{1}{N}\|X\beta-Y^*\|_2^2 + R_N(\beta)\right\}. \label{eq:ols-sgd}
\end{equation}
In the current form, the SGD-OLS estimator could be viewed as a solution of the regularized learning problem with the true loss of OLS as the objective and $R_N(\beta)$ as the regularizer. Though $\mathbb{E}[R_N(\beta)]=0$, we are interested in the implicit regularization effects of the term when $N$ is finite. 
\end{proposition}

\begin{assumption}[Bounded Variances and Bounded Responses] We assume the data samples are all well-normalized, such that for any $1\leq i\leq N$ and $\forall\beta\in\mathcal{C}$, there has $\sigma^2_i\leq M_1$ and $|x_i^\top\beta|\leq M_2$, where $M_1$ and $M_2$ are two constants.
\end{assumption}


\begin{proposition}[Bound of $R_N(\beta)$ with finite $N$]  In a probability higher than $1-2\eta$, there has
\begin{equation}
    - \frac{2}{N}\sqrt{\mathrm{log}\frac{1}{\eta} \sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2} \leq R_N(\beta) \leq \frac{2}{N}\sqrt{\mathrm{log}\frac{1}{\eta} \sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2}\ ,\label{eq:up-bound}
\end{equation}
under mild conditions. With bounded $\sigma_i$ and $x_i^\top\beta$ for $1\leq i\leq N$, there has $R_N(\beta)\to 0$ as $N\to\infty$ and the asymptotic rate of convergence is
\begin{equation}
\left|R_N(\beta)\right|\leq 2M_2\sqrt{\mathrm{log}\frac{1}{\eta}\ \frac{M_1}{N}}
\end{equation}
in a high probability.
\end{proposition}

\begin{proof}
We denote $\varepsilon'_i=-\varepsilon_i$ for $1\leq i\leq N$, then we have  $\mathbb{E}(\varepsilon'_i)=0$ $\mathrm{var}(\varepsilon'_i)=\sigma_i^2$. We further assume $\varepsilon_i$ (so as $\varepsilon'_i$) is well bounded, such that for some positive real $L$ and every integer $k>1$ there has
\begin{equation}
    \mathbb{E}\ \left|(\varepsilon_i x_i^\top\beta)^k\right|\leq\frac{1}{2}\mathbb{E}\ (\varepsilon_i x_i^\top\beta)^2 {L}^{k-2} k!\ .
\end{equation}
So as to the form based on $\varepsilon'_i$, such that
\begin{equation}
    \mathbb{E}\ \left|(\varepsilon'_i x_i^\top\beta)^k\right|\leq\frac{1}{2}\mathbb{E}\ (\varepsilon'_i x_i^\top\beta)^2 {L}^{k-2} k!\ .
\end{equation}
Under the assumption of independence, we could extend the Bernstein's inequality to the form such that
\begin{equation}
    \mathbb{P}\left(\sum_{i=1}^N\varepsilon_i x_i^\top\beta\leq 2t\sqrt{\sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2} \right)\geq 1-\mathrm{exp}(-t^2),
\end{equation}
for $0\leq t\leq \frac{1}{2L}\sqrt{\sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2}$. So as to the form based on $\varepsilon'_i$, such that 
\begin{equation}
    \mathbb{P}\left(\sum_{i=1}^N\varepsilon'_i x_i^\top\beta\leq 2t\sqrt{\sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2} \right)\geq 1-\mathrm{exp}(-t^2),
\end{equation}
for $0\leq t\leq \frac{1}{2L}\sqrt{\sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2}$. Finally, we set $\mathrm{exp}(-t^2)=\eta$, then $t=\sqrt{\mathrm{log}(1/\eta)}$. We consider the bounds from both sides hold independently and the probability should be at least $(1-\eta)^2\geq 1-2\eta$. We complete the proof. \hfill$\square$
\end{proof}

%\begin{proposition}[Nonconvex Minimax Estimator] We consider \textbf{Proposition 2} (in Eq~\ref{eq:up-bound}) with OLS estimator (in Eq~\ref{eq:ols-sgd}) and rewrite SGD-based OLS estimator as a minimax estimator in higher probabilities, such that
%\begin{equation}
%    \widehat\beta_\mathrm{OLS}^\mathrm{SGD}\gets\underset{\beta\in\mathbb{R}^d}{\mathrm{argmin}}\left\{\underset{\sigma_1\dots\sigma_N}{\mathrm{max}}\  \left(\frac{1}{N}\|X\beta-Y^*\|_2^2 - \frac{2}{N}\sqrt{\mathrm{log}\frac{1}{\eta} \sum_{i=1}^N\sigma_i^2(x_i^\top\beta)^2}\right)\right\}. \label{eq:minimax}
%\end{equation}
%The loss function appeared in Eq~\ref{eq:minimax} is nonconvex and could ensure minimax estimate in a high probability.
%\end{proposition}

